#TulsaFlop: A Case Study of Algorithmically-Influenced Collective Action on TikTok

When a re-election rally for the U.S. president drew smaller crowds than expected in Tulsa, Oklahoma, many people attributed the low turnout to collective action organized by TikTok users. Motivated by TikTok's surge in popularity and its growing sociopolitical implications, this work explores the role of TikTok's recommender algorithm in amplifying call-to-action videos that promoted collective action against the Tulsa rally. We analyze call-to-action videos from more than 600 TikTok users and compare the visibility (i.e. play count) of these videos with other videos published by the same users. Evidence suggests that Tulsa-related videos generally received more plays, and in some cases the amplification was dramatic. For example, one user's call-to-action video was played over 2 million times, but no other video by the user exceeded 100,000 plays, and the user had fewer than 20,000 followers. Statistical modeling suggests that the increased play count is explained by increased engagement rather than any systematic amplification of call-to-action videos. We conclude by discussing the implications of recommender algorithms amplifying sociopolitical messages, and motivate several promising areas for future work.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> deleted.tex <==
\subsubsection{Algorithmic Visibility}
Finally, the overall and user-specific visibility analysis informed a scheme for classifying algorithmic visibility. This was intended to answer: which videos received high algorithmic visibility on TikTok? We created four clusters of algorithmic visibility based on an overview of the recommender system's interworkings \cite{wang2020algorithm} which detailed four steps in the distribution pipeline: (1) a cold start with limited distribution, (2) engagement-based distribution, (3) distribution to user groups, and (4) mass distribution to the trending pool. The author of the overview noted that these four steps were based on presentations by the chief engineer at ByteDance (TikTok's parent company), however, these still reflect a general framework for understanding the pipeline, and the actual pipeline currently used by TikTok may differ.


Based on the patterns observed in the overall visibility analysis, we assigned each video to a logarithmic bin according to play count: 1-100 plays, 100-1,000 plays, 1,000-10,000 plays, 10,000-100,000 plays, or 1 million+ plays.



With video statistics for a single user, it is straightforward to infer which of the user's videos were frequently recommended in TikTok's For You pages, and thus received high algorithmic visibility. For example, consider videos from one account that promoted collective action, depicted in Figure \ref{fig:maryjo_videos}. As of early July, one video (about registering for rally tickets) had been played over 2 million times, and fewer than 18,000 users followed the account. We can thus infer this video was frequently recommended by TikTok's "For You" algorithm, as it could not have received all its views "organically" from followers.



After inferring a user's video received high algorithmic visibility in TikTok's recommender system, we then measured the approximate \textit{extent} to which the video was amplified. To do this, we collected up to 500 recent videos published by each user, and compared the visibility of these videos to the visibility of the videos promoting collective action. We did this using two baselines: (1) user-specific central tendency measures and (2) "success clusters" based on the full dataset.


\subsubsection{Central Tendency Baselines}
First, we used simple measures of central tendency to calculate baselines for each user. These baselines were simply the average number of plays, the median number of plays, and the modal number of plays bucketized by thousands of views (i.e. 0-1,000 views, 1,000-2,000 views, etc.).


\subsubsection{Success Clusters Baseline}
For the success clusters baseline, we used agglomerative clustering on the number of plays to assign each video into four levels of distribution. The four groups were based on an overview the recommender system's interworkings \cite{wang2020algorithm}, which detailed four steps in the distribution pipeline: (1) a cold start with limited distribution, (2) engagement-based distribution, (3) distribution to user groups, and (4) mass distribution to the trending pool. The author of the overview noted that these four steps were based on presentations by the chief engineer at ByteDance (TikTok's parent company), however, these still reflect a general framework for understanding the pipeline, and the actual pipeline currently used by TikTok may differ.



%Following recent calls to demonstrate fragility or robustness of findings via multiple analyses, their findings \cite{dragicevic2019increasing}, we constructed two models. The second model was intended to glimpse the relative importance of different factors that affect video visibility on the platform. TikTok has stated that their recommender system weights factors differently when personalizing the "For You" feed \cite{tiktok2020foryou}, but has not explained their relative weights beyond saying that some factors are "weak signals" (e.g., language preference) and some are "strong signals" (e.g., watching a video to the end) \cite{wang2020algorithm}. While our data can only capture some of these signals, a model that uses these variables can still suggest which factors matter to the recommender more than others for predicting play count.

% Due to multicollinearity (i.e. linear dependence among independent variables), we created an "engagement score" variable for the second model, intending to preserve both predictability and interpretability. The "engagement score" was a weighted linear combination of like count, share count, and comment count. In this score, one like was worth one point, one share was worth 41 points, and one comment was worth 56 points. The weights for shares (and comments) were determined by the ratio of total likes to total shares (and likes to comments) across the whole dataset.

%We used three approaches to create an initial sample of users who made videos that suggested registering for the Tulsa rally. The initial three approaches included: (1) a set of TikTok videos compiled by journalist Jenna Amatulli , (2) hashtags associated with the demonstration, namely \#EmptySeats and \#TulsaFlop \cite{wells2020tiktok}, and (3) soundtracks from the seed videos which were used as audio in subsequent videos (i.e. "challenges"). This set provided 619 relevant videos published before June 20th (the date of the rally).

%While 19\% of users in our dataset had at least one video with more than 100,000 plays, less than 1\% of users received more than 100,000 plays on their Tulsa-related video. Using linear models to explain the drivers of play count, we found that users' follower count only explained 1\% of the variation in video play count, while video-specific engagement (i.e. likes, comments, and shares) explained over 87\% of the variation. Given this outsized influence of the recommender algorithm in comparison to social connections, we develop a method for classifying algorithmic visibility on TikTok.
